CLIP-AD: A Language-Guided Staged Dual-Path Model for Zero-shot Anomaly Detection

This paper considers zero-shot Anomaly Detection (AD), performing AD without reference images of the test objects. We propose a framework called CLIP-AD to leverage the zero-shot capabilities of the large vision-language model CLIP. Firstly, we reinterpret the text prompts design from a distributional perspective and propose a Representative Vector Selection (RVS) paradigm to obtain improved text features. Secondly, we note opposite predictions and irrelevant highlights in the direct computation of the anomaly maps. To address these issues, we introduce a Staged Dual-Path model (SDP) that leverages features from various levels and applies architecture and feature surgery. Lastly, delving deeply into the two phenomena, we point out that the image and text features are not aligned in the joint embedding space. Thus, we introduce a fine-tuning strategy by adding linear layers and construct an extended model SDP+, further enhancing the performance. Abundant experiments demonstrate the effectiveness of our approach, e.g., on MVTec-AD, SDP outperforms the SOTA WinCLIP by +4.2/+10.7 in segmentation metrics F1-max/PRO, while SDP+ achieves +8.3/+20.5 improvements.

==> sec/tables/rebuttal_attention.tex <==
\begin{tabular}{@{}l|ccccccc@{}}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{4}{c}{Segmentation} & \multicolumn{3}{c}{Classification}\\
    \cmidrule(r){2-5}
    \cmidrule(r){6-8}
    ~ & AUROC & F1 & AP & PRO & AUROC & F1 & AP \\
    \midrule
    Q-Q & 83.8 & 15.9 & 11.3 & 63.9 & 77.1 & 78.4 & 80.1 \\
    K-K & \underline{86.3} & \underline{16.7} & \underline{12.0} & \textbf{68.9} & \underline{77.9} & \underline{78.8} & \underline{80.5} \\
    V-V &  \textbf{88.1} & \textbf{17.0} & \textbf{12.2} & \underline{68.4} & \textbf{78.6} & \textbf{79.2} & \textbf{81.5} \\
    \bottomrule
  \end{tabular}

==> sec/tables/rebuttal_less_data.tex <==
\begin{tabular}{@{}l|ccccccc@{}}
    \toprule
    Train & \multicolumn{4}{c}{Segmentation} & \multicolumn{3}{c}{Classification}\\
    \cmidrule(r){2-5}
    \cmidrule(r){6-8}
    Data & AUROC & F1 & AP & PRO & AUROC & F1 & AP \\
    \midrule
    \textbf{1/10} & 90.4 & 38.5 & 33.7 & 83.7 &  91.0 & 93.0 & 95.8 \\
    \textbf{All} & 91.2 & 40.0 & 36.3 & 85.1 & 92.2 & 93.4 & 96.6 \\
    \bottomrule
  \end{tabular}

==> sec/tables/rebuttal_opposite.tex <==
\begin{tabular}{@{}l|ccccccc@{}}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{4}{c}{Segmentation} & \multicolumn{3}{c}{Classification}\\
    \cmidrule(r){2-5}
    \cmidrule(r){6-8}
    ~ & AUROC & F1 & AP & PRO & AUROC & F1 & AP \\
    \midrule
    Inversion & 78.4 & 18.6 & 13.5 & 59.8 & 78.0  & 86.4 & 90.6 \\
    DBSCAN & \textbf{87.5} & \textbf{35.9} & \textbf{30.4} & \textbf{75.3} & \textbf{90.9} & \textbf{91.9} & \textbf{95.8} \\
    \bottomrule
  \end{tabular}

==> sec/tables/rebuttal_rep_vec.tex <==
\begin{tabular}{@{}l|ccccccc@{}}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{4}{c}{Segmentation} & \multicolumn{3}{c}{Classification}\\
    \cmidrule(r){2-5}
    \cmidrule(r){6-8}
    ~ & AUROC & F1 & AP & PRO & AUROC & F1 & AP \\
    \midrule
    5Vecs (PCA) & 74.8 & 23.4 & 16.9 & 56.6 & 83.6 & 88.7 & 92.6 \\
    KernelPCA & 86.2 & \textbf{36.1} & \underline{30.2} & \underline{74.4} & \underline{90.7} & \underline{91.9} & \textbf{95.8} \\
    GMM & \underline{86.7} & 35.6 & 29.4 & 74.2 & \underline{90.7} & \textbf{92.2} & \underline{95.7} \\
    DBSCAN & \textbf{87.5} & \underline{35.9} & \textbf{30.4} & \textbf{75.3} & \textbf{90.9} & \underline{91.9} & \textbf{95.8} \\
    \bottomrule
  \end{tabular}
